Mixture of multilayer stochastic block models for multiview clustering

In this work, we propose an original method for aggregating multiple clustering coming from different sources of information. Each partition is encoded by a co-membership matrix between observations. Our approach uses a mixture of multilayer Stochastic Block Models (SBM) to group co-membership matrices with similar information into components and to partition observations into different clusters, taking into account their specificities within the components. The identifiability of the model parameters is established and a variational Bayesian EM algorithm is proposed for the estimation of these parameters. The Bayesian framework allows for selecting an optimal number of clusters and components. The proposed approach is compared using synthetic data with consensus clustering and tensor-based algorithms for community detection in large-scale complex networks. Finally, the method is utilized to analyze global food trading networks, leading to structures of interest.

==> Annexe/Notations.tex <==
\newpage


\section{Notations}
%\vspace{-0.5cm}
\begin{equation*}
\begin{aligned}
\begin{aligned}
%% Variables - nombres
N &\qquad  \text {Number of observations} \\
V &\qquad  \text {Number of views} \\
K &\qquad  \text {Number of clusters} \\
Q &\qquad  \text {Number of sources in the mixture of views} \\
%% Indiçage
i,j &\qquad  \text {Indexes on observations, } i,j \in \left\{1,\dots, N\right\}\\
v &\qquad  \text {Index on views, } v \in \left\{1,\dots, V\right\}\\
k,l &\qquad  \text {Indexes on clustering, } k,l \in \left\{1,\dots, K\right\}\\
s &\qquad  \text {Index on sources, } s \in \left\{1,\dots, Q\right\}\\
%% Variables aléatoires
\textbf{A} &\qquad  \text{Multilayer tensor adjacency } (N \times N \times V)  \\
\textbf{Z} &\qquad  \text{Matrix of clustering latent variables} \\
\textbf{W} &\qquad  \text{Matrix of sources latent variables} \\
\boldsymbol{\rho} &\qquad  \text{Vector of clustering proportions} \\
\boldsymbol{\pi} &\qquad  \text{Vector of proportions in the mixture of views} \\
\boldsymbol{\alpha} &\qquad  \text{component-connection probability parameters tensor} \\
%% Paramètres variationnels
\boldsymbol{\tau} &\qquad  \text{Variational paramater for } \textbf{Z}  \\
\boldsymbol{\nu} &\qquad  \text{Variational paramater for } \textbf{W} \\
%% Paramètres bayesiens
\boldsymbol{\beta}^0 &\qquad  \text{Hyper-parameter of Bayesian model, for community components } \\
\boldsymbol{\theta}^0 &\qquad  \text{Hyper-parameter of Bayesian model, for view components} \\
\boldsymbol{\eta}^0 , \boldsymbol{\xi}^0 &\qquad  \text{Hyper-parameter of Bayesian model, for connection tensor} \\
%% Lois et fonctions
\p &\qquad  \text{True distribution} \\
q &\qquad  \text{Variational distribution} \\
\mathcal{B} &\qquad  \text{Bernoulli distribution} \\
\mathcal{M} &\qquad  \text{Multinomial distribution} \\
\dir &\qquad  \text{Dirichlet distribution} \\
\bet &\qquad  \text{Beta distribution} \\
\Gamma &\qquad  \text{Gamma function} \\
\psi &\qquad  \text{Digamma function} \\
\KL &\qquad  \text{Kullback-Leibler divergence} \\
\end{aligned}
\end{aligned}
\end{equation*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% Networks provide a powerful and intuitive way to represent complex systems of relationships between individuals. They provide a effective and informative representation of the system.

% To represent the graph structure, the adjacency matrix associated to this graph $\bA$ can be used. $\bA$ is a square matrix, and its entries represent the strength of the connections between nodes.

% For a undirected binary graph, $\bA$ is symmetric and each entry indicates if there is an edge between nodes or not. In case of connection between $i$ and $j$, the $(i,j)$ and $(j,i)$ entries will both be $1$, or $0$ else.

% In clustering framework, the output of algorithms are often a classification, or a membership matrix. This information, although useful, has the drawback of depending very strongly on the number of clusters chosen when using the algorithm. To erase this problem, this output can be transform into an adjacency matrices by : 
% \begin{equation*}
% \label{adjacencySBM}
%     {A}_{ij}=
%     \begin{cases}
%       1, & \text{if}\ \text{individuals $i$, $j$ are linked in the same cluster}, \\
%       0, & \text{otherwise}.
%     \end{cases}
% \end{equation*}

% % Model based approach of clustering aggregation
% The process of combining numerous data clusters that have already been discovered using various clustering algorithms or approaches is known as meta-clustering. Finding connections and similarities across clusters that might not be immediately obvious when looking at them separately is the aim of meta-clustering.
% Model-based meta-clustering offer advantages: knowing the redundancy of information sources and their complementarity, obtaining a final clustering from all the clustering outputs already carried out, allowing the best possible grouping of individuals through different information sources.
% Moreover, model-based meta-clustering allow to have an evaluation criterion on the performance of the model (e.g. log-likelihood, evidence, etc.) and, at least in the Bayesian framework, criteria for model selection. 

==> biblio.tex <==
% ---- Bibliography ----
%
% BibTeX users should specify bibliography style 'splncs04'.
% References will then be sorted and formatted in the correct style.
%
% \bibliographystyle{splncs04}
% \bibliography{mybibliography}
%



% \begin{thebibliography}{8}
% \bibitem{ref_article1}
% Author, F.: Article title. Journal \textbf{2}(5), 99--110 (2016)

% \bibitem{ref_lncs1}
% Author, F., Author, S.: Title of a proceedings paper. In: Editor,
% F., Editor, S. (eds.) CONFERENCE 2016, LNCS, vol. 9999, pp. 1--13.
% Springer, Heidelberg (2016). \doi{10.10007/1234567890}

% \bibitem{ref_book1}
% Author, F., Author, S., Author, T.: Book title. 2nd edn. Publisher,
% Location (1999)

% \bibitem{ref_proc1}
% Author, A.-B.: Contribution title. In: 9th International Proceedings
% on Proceedings, pp. 1--2. Publisher, Location (2010)

% \bibitem{ref_url1}
% LNCS Homepage, \url{http://www.springer.com/lncs}. Last accessed 4
% Oct 2017
% \end{thebibliography}

==> multimodale/multimodale_data.tex <==
\section{Background}


In  multiview clustering, various fusion strategies have been devised to effectively combine information from different sources of information. One possible taxonomy of these strategies is related to the timing of fusion: early, intermediate or late. \textit{Early fusion} starts by merging the different view before clustering. \textit{Intermediate fusion} considers the integration of views within the clustering algorithm. \textit{Late fusion} consists in clustering each view separately and then integrating all the resulting partitions into a unique integrated clustering. This paper focuses on late  multiview clustering.  In this senario, all layers represented as adjacency matrices collectively form a tensor.

This latter strategy harnesses the benefits of employing specific and well-suited clustering approaches for each view and takes advantage of their complementarity and redundancies by merging their results in a subsequent phase. In this context, \textit{consensus clustering} serves as a baseline and will be first described in this section. 
%
On the other hand, \textit{latent} or \textit{stochastic block models} provide advantageous characteristics for multiview clustering in term of model selection. In this section, we will also provide a focused overview of these approaches, to which our method, tailored to late fusion clustering, belongs.

%Our proposed method falls within these approaches by adapting them to the context of late fusion. In this section, we will also provide a selective presentation of these approaches.

% An typical strategy in late fusion processes is \textit{consensus clustering} which will be regarded as a baseline in this paper. On the other hand, convenient properties  %\textcolor{orange}{bonnes proprietes de modelisation} 
% in multiview problems and can be adapted to late fusion purposes.



% \subsection{Late Multimodal Clustering}

% Multimodal clustering gathers data into distinct groups by utilizing complementary information from multiple modalities or views. This problem may also be related to data fusion or data integration according to the field of application. 



% Typical approaches in this category are  Consensus clustering and Tensor-based meta-clustering.  



\subsection{Consensus clustering}

% \MS{message: }{consensus clustering as a baseline for data representation}

% \CA{Intro }{\textit{Consensus clustering} is a family of methods which are based on the construction of a consensus matrix that represents the degree of agreement among different clustering algorithms, as in~\cite{montiConsensusClusteringResamplingBaseda}.  
% Each element of the matrix represents the frequency with which nodes are clustered together across different clustering runs. Several methods have been developed, and in particular the Monte Carlo reference-based consensus clustering (M3C) \citep{montiConsensusClusteringResamplingBaseda} that combines multiple clustering solutions generated by applying different clustering algorithms and parameters to the same dataset and utilizing random sampling and resampling techniques.}

Consensus clustering \citep{montiConsensusClusteringResamplingBaseda,fred2005combining},  also known as cluster ensemble \citep{strehl2002cluster, golalipour2021clustering}, is a technique used to find a single partition from multiple clustering solutions. 

It is used to integrate and analyze multiple clustering results obtained from different algorithms, parameter settings, or subsets of the data. It aims to find a consensus or agreement among the individual clustering solutions to obtain a more robust and reliable clustering result. Consensus clustering is like asking for multiple opinions (clusters) and then finding a common answer (consensus) that represents an overall agreement.

Each run generates a set of clusters, which can be represented as a partition matrix where each entry indicates the cluster assignment of each data point. An agreement matrix is constructed from all the partition matrices. The entries in this matrix indicate the frequency with which pair of data points co-occur in the same cluster across all solutions.
The final clusters are determined by applying a clustering algorithm %(like hierarchical clustering) 
on the agreement matrix. 

%Several methods have been developed, and 
In particular, the Monte Carlo reference-based consensus clustering (M3C) \citep{montiConsensusClusteringResamplingBaseda} combines multiple clustering solutions generated by applying different clustering algorithms and parameters to the same dataset using random (re)sampling techniques.

%\subsection{Multi$\star$ Block Models}
\subsection{Block models for multiview clustering}

% \CA{Intro}{\textit{Tensor-based meta-clustering} utilizes %tensor 
% multilinear algebra decomposition techniques to identify patterns and relationships across each layer of this tensor ;  in case of meta-clustering, all layers are often adjacency matrices, as in~\citep{jingCommunityDetectionMixture2020a}.   %(e.g. \textit{TWIST} algorithm \cite{jingCommunityDetectionMixture2020a}). 
% In the literature, there are often two approaches used : The Tucker decomposition, which divides a tensor into a core tensor and a collection of factor matrices that depict the connections between the tensor modes, like \textit{TWIST} algorithm ~\citep{jingCommunityDetectionMixture2020a} or \textit{ALMA} algorithm ~\citep{fan2021alma} , and the canonical decomposition that breaks down a tensor into a collection of orthogonal factor matrices that describe the underlying modes of variation in the data.
% Finally, \textit{Mixture Multilayer Stochastic Block Models} (MMSBM) 
% expands the traditional SBM by considering multilayer networks, allowing the layers to come from a mixture model, as in ~\citep{fan2022alma} or ~\citep{rebafka2023modelbased}. 
% However,  often, in this type of model there is a classification of individuals within each view component, giving only an idea of the clustering when conditioning the chosen view. In the other hand, MMSBM can be used in conjunction with other learning methods, such as hierarchical classification, like \textit{graphclust}~\citep{rebafka2023modelbased}, or tensor decomposition~\citep{jingCommunityDetectionMixture2020a,fan2021alma,noroozi2022sparse}, to obtain higher performance or robustness.}

%\paragraph{Context.}


With a wide expanse of literature existing on this subject, we narrow our focus toward studies in which the distinct views represent varying types of interactions among a common set of $N$ observations. However, it's important to note that our scope excludes studies that aim to establish partitions with overlaps or mixed memberships, as well as those where views show specific dependencies (spatial or temporal for instance).
Works of this nature can be discovered in the references provided below.


%There is a substantial literature dedicated to %latent and 
%stochastic block models in multiview learning. 
In the framework of block models for multiview clustering, the views are commonly denoted as a collection of $V$ \textit{graphs} or more often as $V$ \textit{layers} within a single network, and the terminologies of  \textit{multigraph}, \textit{multilayer} or even \textit{multiplex} may be employed. The initial approaches were focused on identifying a partition  $\bZ$ with $K$ blocks of observations that encompass the different layers. More recent studies establish structural patterns within individual layers as well as across multiple layers, resulting in the generation of multiple partitions of observations, along with an additional layer-level organizational structure.
% More recent studies  assume that a structure can be established both within and across the distinct layers, leading to $V$ partitions $\bZ^{(v)}$ and an
% additional organization for the layers.

%\begin{rem}
% %The literature surrounding this topic is vast. Therefore, we direct our attention 
% With a wide expanse of literature existing on this subject, we narrow our focus towards studies in which the distinct views represent varying types of interactions among a common set of $N$ observations. However, it's important to note that our scope excludes studies that aim to establish partitions with overlaps or mixed memberships, as well as those where layers show specific (spatial or temporal for instance) dependencies.
% \MS{Out of scope:}{works with overlapping / mixed memberships (MMSBM) and spatial / temporal layers dependencies}\\
% +\\
% \MS{Huge literature around the subject:}{\textbf{selective} review}
%\end{rem}

\subsubsection{Multilayer SBM} 

% \MS{Blabla:}{MultiLayer SBM (MLSBM) for finding a block partition across  multiple layers with VEM or spectral clustering}
A popular kind of inference for block models estimation relies on Variational Expectation Maximization (VEM) algorithms ~\citep{daudin2008mixture}. When the data originate from a multilayer SBM (MLSBM), different estimation techniques can also be applied to identify the partition. Out of these, 
spectral clustering finds widespread usage.~\citep{von2007tutorial, von2008consistency}

\paragraph{VEM inference.} 
In this setting, different SBM based approaches have been proposed for %multigraphs~\citep{holland1983stochastic}, 
multilayer~\citep{han2015consistent, subhadeep2016consistent} or similarly for multiplex~\citep{barbillon2017stochastic} networks. \cite{han2015consistent} 
%explore the asymptotic properties of class memberships when the number of relations grows for spectral clustering and also
propose a consistent maximum-likelihood estimate (MLE) and explore the asymptotic properties of class memberships when the number of relations grows. \cite{subhadeep2016consistent} also study the consistency 
of two other MLEs when the number of nodes or the number of types of edges grow together. \cite{barbillon2017stochastic}  introduce an Erd\"{o}s-Rényi model that may also integrate covariates related to pairs of observations and use an Integrated Completed Likelihood (ICL)~\cite{biernacki2010exact} %MS{criterion}{[cite]} 
for the purpose of model selection. Also based on VEM estimation, the work of~\cite{boutalbi2021implicit} is grounded on Latent Block Models (LBM). 


%Exploring different integration schemes opens the door to using alternative estimation methods as well. 
\paragraph{Spectral clustering.}   
%For instance, %\cite{valles2016multilayer} merge the multiple layers of a network using logical \texttt{AND} or \texttt{OR} mechanisms and address an aggregated SBM problem. 
Here, we shed light on several extensive research efforts focused on spectral clustering under the assumption of data generated by a Multilayer Stochastic Block Model.  \cite{han2015consistent} investigate the asymptotic characteristics related to spectral clustering. \cite{chen2017multilayer} introduce a framework for multilayer spectral graph clustering that includes a scheme for adapting layer weights, while also offering statistical guarantees for the reliability of clustering. \cite{mercado2018power} presents a spectral clustering algorithm for multilayer graphs that relies on the matrix power mean of Laplacians. \cite{paul2020spectal} show the consistency of the global optimizers of co-regularized spectral clustering and also for the orthogonal linked matrix factorization. Finally, \cite{huang2022spectral} propose integrated spectral clustering methods based on convex layer aggregations.

\paragraph{Limits.} \MS{Limits:}{patterns in layers.}

% S. Heimlicher, M. Lelarge, and L. Massouli ́e. Community detection in the labelled stochastic block model. arXiv:1209.2910, 2012.
% [58] J. Xu, L. Massouli, and M. Lelarge. Edge label inference in generalized stochastic block models: from spectral theory to impossibility results. In COLT, 2014.
%[59] M. Xu, V. Jog, and P.-L. Loh. Optimal rates for community estimation in the weighted stochastic block model. arXiv:1706.01175, 2017.
%[60] S.-Y. Yun and A. Proutiere. Optimal cluster re- covery in the labeled stochastic block model. In NIPS. 2016.
% [23] H.-C. Huang, Y.-Y. Chuang, and C.-S. Chen. Affinity aggregation for spectral clustering. In CVPR, 2012.
% [24] V. Jog and P.-L. Loh. Information-theoretic bounds for exact recovery in weighted stochas- tic block models using the Renyi divergence. arXiv:1509.06418, 2015.

%\paragraph{TBMs for finding structures through observations and layers}
%\paragraph{SBMs and TBMs for multiway structures}
\subsubsection{Multiway block models} 

In contrast to the works presented above, where the aim is to establish a partition across the observations, the approaches presented below focus on establishing multiway structures, especially between- and within-layer partitions. In this context, the MLSBM can evolve into either a Mixture of Multilayer SBM (MMLSBM) or expand into a Tensor Block Model (TBM), depending on the specific research communities and their focus.
%the MLSBM may turn into a Mixture of Multilayer SBM (MMLSBM) or extend to a Tensor Block Model (TBM) depending on research communities.

\paragraph{Mixture of multilayer SBM.} \cite{stanley2016clustering} introduced one of the first approaches that integrated a multilayer SBM with a mixture of layers, using a two-step greedy inference method. In the initial step, it infers a  SBM for each layer and groups together SBMs with similar parameters. In the second step, these outcomes serve as the starting point for an iterative procedure that simultaneously identifies $Q$ strata spanning the $V$ layers. In each stratum $s$, the nodes are independently distributed into $K_s$ blocks, leading to $Q$ membership matrices $\{\bZ^1, \cdots, \bZ^Q\}$. 
%where the nodes  $K_s$ blocks of observations within each component.  
%
In pursuit of the same goal, \cite{fan2022alma} develop an alternating minimization algorithm that offers theoretical guarantees for both between-layer and within-layer clustering errors. 
\cite{rebafka2023modelbased} proposes a Bayesian framework for a finite mixture of MLSBM and employs a hierarchical agglomerative algorithm for the clustering process. It initiates with individual singleton clusters and then progressively merges clusters of networks according to 
with an ICL criterion also used 
for model selection. 
%

Also, \cite{pensky2021clustering} presents a versatile model for diverse multiplex networks, including both MLSBM and MMLSBM. However, in the latter scenario, they make the assumption that the number of blocks within each group of layers remains consistent, such that $K_s=K$, $\forall s$. They perform a spectral clustering on the layers and then aggregate the resulting block connectivity matrices to determine the between-layer partition of observations. Using this model as a foundation,\cite{noroozi2022sparse} introduces a more efficient resolution technique rooted in sparse subspace clustering~\citep{elhamifar2013sparse}. They demonstrate that this algorithm consistently achieves strong between-layer clustering results.


\paragraph{Tensor block models.}  A different strategy for addressing the challenge of late fusion multiview clustering involves tensorial modeling and estimation techniques. In the first category, \cite{wang2019multiway} position their research within the context of higher-order tensors. They introduce a least-square estimation method for (sparse) TBM and demonstrate the reliability of block structure recovery as the data tensor's dimension increases by providing consistency guarantees. \cite{han2022exact} suggest employing high-order spectral clustering as an initialization of a high-order Lloyd algorithm. They establish convergence guarantees and statistical optimality under the assumption of sub-Gaussian noise. 
%
\cite{boutalbi2020tensor} introduce an extension of Latent Block Models to handle tensors. They consider multivariate normal distributions for continuous data and Bernoulli distributions for categorical data, implementing a VEM algorithm for this purpose. 
%
Finally, \cite{jingCommunityDetectionMixture2020a} identifies patterns and relationships between and across layers with multilinear algebra tools based on regularized Tucker decomposition. On a first place,  . They also propose a to achieve global partition

\MS{Limits:}{In practice, $K_m = K$ or $K_m$ is known}
% If one is unsure that each of the layers of the network has the same number of communities, one can use a different number of communities K(l)
% in each layer. After groups
% of layers are identified, the number of layers in each group should be re-adjusted, so that
% K(l) = Km if m = c(l). One can, of course, assume that the values of Km, m = 1, ..., M,
% are known. However, since group labels are interchangeable, in the case of non-identical
% subspace dimensions (numbers of communities), it is hard to choose, which of the values
% correspond to which of the groups. This is actually the reason why Jing et al. (2021) and
% Fan et al. (2022), who imposed this assumption, used it only in theory while their simulations and real data examples are all restricted to the case of equal Km, m = 1, ..., M.
% On the contrary, knowledge of K(l) allows one to deal with different ambient dimensions
% (number of communities) in the groups of layers in simulations and real data examples.}

\begin{enumerate}
   \item \textbf{Tensors approcahes}: a huge literature, among them:
\begin{itemize}
    \item \textbf{tensor decompo with MLSBM data generation:} TWIST, ALMA (done below)
    \item \textbf{spectral:}  (\citep{pensky2021clustering} and \citep{noroozi2022sparse}, 
\item \textbf{Tensor-SBMs:} (à lire) 
\cite{han2022exact}, \cite{wang2019multiway}, \cite{boutalbi2020tensor}
\end{itemize}
    \item \MS{\textbf{Mixture of SBMs:}}{DONE !} Tabea \citep{rebafka2023modelbased}, Strata \citep{stanley2016clustering}  + Strata non variationnel ? ALMA ?
\end{enumerate}

\MS{Position of mimi-SBM:}{At the crossroad of MLSBM and MMLSBM -> mixture of layers but a single traversing partition accross the layers}


In the literature, there are often two approaches used. The canonical decomposition that breaks down a tensor into a collection of orthogonal factor matrices that describe the underlying modes of variation in the data. On the other hand, the Tucker decomposition divides a tensor into a core tensor and a collection of factor matrices that depict the connections between the tensor modes. The algorithms \textit{TWIST}~\citep{jingCommunityDetectionMixture2020a} or \textit{ALMA}} belong to the last family.



% Stochastic Block Models (SBMs) are mixture models used to study network data. The nodes are often assumed to belong to different groups or communities, and the SBM models the probability of edges between nodes in different groups. We will describe a special case of SBM for unweighted graphs. Mathematically, this type of SBM can be described as follows:

% we consider an undirected binary random graph $\mathcal{G}$ represented by a $N \times N$ symmetric matrix $\textbf{A}$ where :
% \begin{equation}
% \label{adjacencySBM}
%     {A}_{ij}=
%     \begin{cases}
%       1, & \text{if}\ \text{individuals $i$, $j$ are linked in } \mathcal{G}  \\
%       0, & \text{otherwise}
%     \end{cases}.
% \end{equation}
% Moreover, as it's a mixture model. So, we have latent variables $\textbf{Z}_i$ who describes the group membership, corresponding to the definition in the section \ref{MixtureModel}.

% We can also define $\textbf{Z}$ the indicator matrix of component membership such that $Z_{ik} = 1$ if the individual $i$ belongs to the $k^{th}$ component and $0$ otherwise. 

% SBM models the relationship between individuals based on their membership of the components, and thus with the latent variables. So, SBM models the probability of edge between $i$ and $j$ by :
% \begin{equation}
% A_{ij} | Z_{ik} = 1, Z_{jl} = 1 \sim \mathcal{B}(\alpha_{kl})\\ 
%     %\mathbb{P}(A_{ij} = 1 | Z_{ik}=1, Z_{jl} = 1) = \alpha_{kl},
% \end{equation}
% with $\mathcal{B}(.)$ the Bernoulli distribution, and $\boldsymbol{\alpha}$ a $K\times K$ matrix of component-connection probability.

% For this model, we assume :
% \begin{itemize}
%     \item no self-loop: $A_{ii}$ elements are not considered.
%     \item latent variable are independent : $\textbf{Z}_i \ind \textbf{Z}_j$, $\forall i \ne j$
%     \item edges are independent given latent variables. 
% \end{itemize}


% \subsubsection{Multilayer SBM}

% This mixture model is very efficient to model the link between individuals from graphs, however it has a major flaw. First of all, it considers only one source of information, in its formulation only one graph is taken into account, which limits very strongly the description of the links between individuals. A method allowing to fill this gap, would be simply to add all the matrices of adjacency resulting from each source, and to treat that with the adequate law, but we would arrive at a second concern.
% This approach would treat all sources in the same way, and would put forward the most redundant information, thus the one with the most impact on the structure, without taking into account the particularities of each source of information.



% \subsection{Block models}




